Biased-MPPI: Informing Sampling-Based Model Predictive Control by Fusing Ancillary Controllers

Motion planning for autonomous robots in dynamic environments poses numerous challenges due to uncertainties in the robot's dynamics and interaction with other agents. Sampling-based MPC approaches, such as Model Predictive Path Integral (MPPI) control, have shown promise in addressing these complex motion planning problems. However, the performance of MPPI relies heavily on the choice of sampling distribution. Existing literature often uses the previously computed input sequence as the mean of a Gaussian distribution for sampling, leading to potential failures and local minima. In this paper, we propose a novel derivation of MPPI that allows for arbitrary sampling distributions to enhance efficiency, robustness, and convergence while alleviating the problem of local minima. We present an efficient importance sampling scheme that combines classical and learning-based ancillary controllers simultaneously, resulting in more informative sampling and control fusion. Several simulated and real-world demonstrate the validity of our approach.

==> tex/intro.tex <==
\section{Introduction}\label{sec::intro}
When autonomous robots navigate real-world human-populated environments, they have several difficulties to overcome. For one, uncertainties in the state and model of the robot and the environment, as well as in the interaction and predictions of other agents' future motion, are often non-negligible. Desired behaviors for the autonomous robot, such as goal reaching, collision avoidance, maximum allowed speed, or social interaction rules are typically encoded into complex cost functions and constraints, often resulting in non-linear, non-convex, and even discontinuous problem formulations. Moreover, the environment can change in unexpected ways. When that happens, the autonomous robot should quickly react and adjust its future actions accordingly.
Developing a motion planning algorithm accounting for all of the above is an extremely challenging task, and typically this is dealt with by decomposing the large problem into sub-problems, such as path planning, trajectory planning, and tracking \cite{Paden2016}. These so-called hierarchical approaches often have optimality guarantees on each of the sub-solutions given certain assumptions, but optimality is seldom guaranteed for the overall solution. For example, the trajectory planner might use a simple kinematic model to compute a collision-free local trajectory. Still, the tracking controller might have to deviate from it because of dynamic constraints. However, the tracking controller is often blind to obstacles, and therefore deviating from the planned trajectory might result in a collision.
Trying to avoid overly decomposing and simplifying the overall problem, using model-free Deep Reinforcement Learning (DRL) one might learn a policy offline which directly commands inputs to the autonomous agent given, for example, an obstacle map and a goal location. While such methods can perform very well in environments that are close enough to their training set, generalization is rarely guaranteed.
Complex motion planning problems with uncertainties and arbitrary cost functions can also be posed as stochastic optimal control problems, which can then be formulated into stochastic Hamilton Jacobi Bellman (HJB) equations. However, numerically solving such equations is often difficult given the curse of dimensionality. Recently, solving stochastic optimal control problems by means of sampling has been shown to be a very promising direction.
In pioneering work \cite{Kappen2005, Kappen2007a}, it was shown that for control-affine systems the stochastic HJB equations could be linearized and the solution approximated through sampling thanks to the path integral formulation. In later work \cite{williams_aggressive_2016, Williams2017c}, this path integral method was implemented in a receding horizon fashion giving rise to a sampling-based Model Predictive Controller (MPC) called Model Predictive Path Integral (MPPI) control. A related approach based on information theory was then proposed \cite{Williams2017, Williams2018a}, which removed the assumption on the affinity in control and demonstrated easier applicability to discrete-time systems. This sampling-based MPC approach, thanks to being naturally parallelizable, can be implemented on a GPU and achieve fast control loops and large prediction horizons while solving problems that are potentially non-linear, non-convex, and even discontinuous \cite{Williams2017, Williams2017c}.
MPPI and its Information-Theoretic counterpart have been successfully applied to several different types of systems and problems. Thanks to its fast computations, MPPI was shown to be suitable for racing a small-scale rally car on a dirt track at high-speed \cite{Williams2017, Williams2017c}, also when combined with game theoretic approaches \cite{Williams2018a}. In recent work, MPPI was also applied in simulation to an autonomous car with dynamic obstacles \cite{perez-morales_Information-Theoretic_2021}. With equal success, MPPI was also adapted to fly drones in partially observable environments \cite{mohamed_model_2020}, fly complex maneuvers \cite{Pravitra2021}, and in combination with an adaptive control scheme \cite{pravitra_l1-adaptive_2020}. In some work, MPPI was adapted to multi-agent systems, for example, to fly in formation \cite{Gomez2016} and in cooperation \cite{wan_cooperative_2021}. In particular, a variant of MPPI was recently proposed for interaction-aware collision avoidance in decentralized, non-communicating multi-agent environments (cite lucas). Promising results were also shown for manipulators \cite{bhardwaj_storm_2021}, also when considering model uncertainty in the planning \cite{abraham_model-based_2020}. In particular, given its sampling nature, MPPI can easily deal with discontinuous dynamics such as the ones encountered when a robot arm is tasked with pushing objects \cite{arruda_uncertainty_2017, cong_self-adapting_2020}, or planning motion for a four-legged walking robot \cite{carius_constrained_2021}.
In general, being a model-based approach, MPPI needs a model in order to forward simulate the trajectories given the sampled inputs. In recent work, however, a physics-based engine was used to simulate the samples, thus not requiring the burden of explicitly writing the dynamics of the agents and the environment \cite{carius_constrained_2021}. This advantage is similar to that of reinforcement learning, where one can train a policy in a simulator offline before applying it to the robot. With MPPI however, the samples have to be taken online, which can require more computations than real-time constraints allow for. This issue can be alleviated by using novel GPU-based physics engines which will enable for parallel simulations (cite Isaac). Moreover, it was shown that an ensemble of simulators can be used with MPPI to produce a control input that is robust to uncertainties, behaving conservatively when the uncertainty is high and more aggressively when the uncertainty is low \cite{abraham_model-based_2020}. Adapting model parameters and planning with uncertainty was also explored in \cite{guzman_bayesian_2022}


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.48\textwidth]{images/sampling_problem.png}
    \caption{Problems with using previously computed control sequence as a mean of a Gaussian sampling distribution. Left: large unexpected disturbance kicks a racing car sideways, resulting in all the samples taken crashing into the barriers. Middle: a dynamic obstacle unexpectedly moves in front of us. Taking the previous control input sequence to sample, we do not discover a braking maneuver. Right: two agents cross each other paths while having to avoid collisions. Without a large sampling variance, using the previously computed input easily results in the two robots getting stuck in a local minimum.}
    \label{fig:sampling_fail}
\end{figure}

Despite all these successes, the performances of the MPPI are, being a sampling-based method, highly dependent on the choice of the sampling distribution. Given the real-time constraint of many applications, the number of samples that can be taken at each time step is limited, which makes the efficiency of the importance sampler even more decisive. Most of the literature, starting from seminal work \cite{williams_aggressive_2016}, uses the time-shifted previously computed input sequence as a mean for Gaussian distribution and uses it for sampling at the current iteration, where the variance can be tuned. As depicted in Fig. \ref{fig:sampling_fail}, while this makes sense in most cases, using the previously computed input sequence can lead to catastrophic failures whenever large unexpected disturbances are introduced or the environment changes in unexpected ways, but can also fail to discover lower cost area of the state space by getting trapped in local minima.

In this paper:
\begin{itemize}
    \item We show rigorous derivations describing how one can elegantly change the sampling distribution to an arbitrary distribution while avoiding numerical issues, and provide insights on how doing so affects the overall method.
    \item We propose an efficient importance sampler that uses several simple ancillary controllers simultaneously to take more informative samples, which can also be seen as a scheme for control fusion. 
    \item In experiments, we demonstrate that the proposed sampling scheme is not only more efficient, but also more robust to disturbances, and rapid changes in the environment, and less susceptible to local minima. Moreover, we show that the proposed scheme is able to take suggestions from ancillary controllers and improve on them.
\end{itemize}

In section \ref{sec::prev_work} we provide an overview of the previous work into improving the importance-sampler for sampling-based control. In section \ref{sec::preliminaries}, we briefly summarize the Information-Theoretic approach to MPPI and outline its issues. In section \ref{sec::prop_approach}, we propose an elegant mathematical formulation that is more robust to numerical issues and allows for arbitrary sampling distributions. In section \ref{sec::experiments}, we demonstrate through experiments that using an informed multi-modal sampling distribution improves the importance sampler efficiency, robustness, and convergence. In section \ref{sec::conclusion}, we conclude by giving an outline of the main results described in this paper. 

